Finite Element Error Estimates for Critical Growth Semilinear Problems without Angle Conditions

In this article we consider a priori error and pointwise estimates for finite element approximations of solutions to semilinear elliptic boundary value problems in d>=2 space dimensions, with nonlinearities satisfying critical growth conditions. It is well-understood how mesh geometry impacts finite element interpolant quality, and leads to the reasonable notion of shape regular simplex meshes. It is also well-known how to perform both mesh generation and simplex subdivision, in arbitrary space dimension, so as to guarantee the entire hierarchy of nested simplex meshes produced through subdivision continue to satisfy shape regularity. However, much more restrictive angle conditions are needed for basic a priori quasi-optimal error estimates, as well as for a priori pointwise estimates. These angle conditions, which are particularly difficult to satisfy in three dimensions in any type of unstructured or adaptive setting, are needed to gain pointwise control of the nonlinearity through discrete maximum principles. This represents a major gap in finite element approximation theory for nonlinear problems on unstructured meshes, and in particular for adaptive methods. In this article, we close this gap in the case of semilinear problems with critical or sub-critical nonlinear growth, by deriving a priori estimates directly, without requiring the discrete maximum principle, and hence eliminating the need for restrictive angle conditions. Our main result is a type of local Lipschitz property that relies only on the continuous maximum principle, together with the growth condition. We also show that under some additional smoothness assumptions, the a priori error estimate itself is enough to give pointwise control the discrete solution, without the need for restrictive angle conditions. Numerical experiments confirm our theoretical conclusions.

==> app.tex <==
\appendix
\addtocontents{toc}{\protect\setcounter{tocdepth}{1}}

\section{Some Supporting Results}
\label{app:entire}

In this appendix we assemble some supporting results that we
exploit at various points in the body of the paper, and also
give some generalizations of results appearing in the paper.

%-----------------------------------------------------------------------------
\subsection{The de Giorgi Iterative Lemma}
%-----------------------------------------------------------------------------
In this section, 
we review the de Girogi iterative lemma for proving the 
maximum principle in Theorem~\ref{thm:maximum} in the case of
monotone nonlinearity.
For a proof of this lemma, we refer to~\cite{De-Giorgi.E1957}, \cite[Lemma 4.1.1]{Wu.Z;Yin.J;Wang.C2006} or~\cite[Lemma 12.5]{Chipot.M2009}. 
For completeness, we include the proof below. 
The term ``iterative'' appearing in the name of the de Giorgi method comes 
from an iterative argument used in proving the lemma.
\begin{lemma}
	\label{lm:degiorgi}
	Let $\phi(\cdot)$ be a non-negative and non-increasing function on $[s_{0}, \infty)$ satisfying
	\begin{equation}
	\label{eqn:degiorgi}
		\phi(s) \leqs \left( \frac{A}{s-r}\right)^{\alpha}[\phi(r)]^{\beta},\qquad \forall s>r\geqs s_{0},
	\end{equation}
	for some constant $A>0, \; \alpha >0$ and $\beta>1.$ Then 
	$$
		\phi(s) \equiv 0,\qquad \forall s\geqs s_{0}  +A2^{\beta/(\beta-1)}[\phi(s_{0})]^{(\beta-1)/\alpha}.
	$$
\end{lemma}
\begin{proof}
	Set $s_{k} = s_{0}  + t - \frac{t}{2^{k}}$ for $k=0, 1, 2, \cdots$. Here $t$ is a constant to be determined. From the assumption \eqref{eqn:degiorgi}, we obtain
	$$
		\phi(s_{k+1}) \leqs \left( \frac{A}{s_{k+1} - s_{k}}\right)^{\alpha} [\phi(s_{k})]^{\beta}
		 =\frac{A^{\alpha} 2^{(k+1)\alpha}}{t^{\alpha}}[\phi(s_{k})]^{\beta}.
	$$
	If we can prove the following inequality: 
	\begin{equation}
		\label{eqn:reduction}
			\phi(s_{k}) \leqs r^{k} \phi(s_{0}),
	\end{equation}
	for some constant $r \in (0,1)$ to be chosen, then by letting $k\to \infty$ we obtain
	$\phi(s_{0} + t) =0$ which concludes the proof of the lemma since $\phi$ is non-increasing.
	
	Now we prove \eqref{eqn:reduction} by induction. Suppose \eqref{eqn:reduction} is true for $k$ then
	\begin{eqnarray*}
		\phi(s_{k+1}) &\leqs& \frac{A^{\alpha} 2^{(k+1)\alpha}}{t^{\alpha}}[\phi(s_{k})]^{\beta}\\
		&\leqs& \frac{\phi(s_{0})}{r^{k+1}} \frac{A^{\alpha} 2^{(k+1)\alpha}}{t^{\alpha} r^{k(\beta -1) -1}}[\phi(s_{0})]^{\beta-1}.
	\end{eqnarray*}
	Choose $r = 2^{\alpha/(\beta -1)}$, then 
	$$
	\phi(s_{k+1}) \leqs  \frac{\phi(s_{0})}{r^{k+1}} \frac{A^{\alpha} 2^{\alpha\beta/(\beta -1)}}{t^{\alpha}}[\phi(s_{0})]^{\beta-1}.
	$$
	From this, \eqref{eqn:reduction} is valid for $s+1$ if $\frac{A^{\alpha} 2^{\alpha\beta/(\beta -1)}}{t^{\alpha}}[\phi(s_{0})]^{\beta-1}\leqs 1$, that is,  we should choose 
	$$
		t\geqs A2^{\beta/(\beta-1)}[\phi(s_{0})]^{(\beta-1)/\alpha}.
	$$
	This concludes the proof.
\end{proof}


